Optimize Incompatible Parameters through Compatibility-aware Knowledge Integration

Deep neural networks have become foundational to advancements in multiple domains, including recommendation systems, natural language processing, and so on. Despite their successes, these models often contain incompatible parameters that can be underutilized or detrimental to model performance, particularly when faced with specific, varying data distributions. Existing research excels in removing such parameters or merging the outputs of multiple different pretrained models. However, the former focuses on efficiency rather than performance, while the latter requires several times more computing and storage resources to support inference. In this paper, we set the goal to explicitly improve these incompatible parameters by leveraging the complementary strengths of different models, thereby directly enhancing the models without any additional parameters. Specifically, we propose Compatibility-aware Knowledge Integration (CKI), which consists of Parameter Compatibility Assessment and Parameter Splicing, which are used to evaluate the knowledge content of multiple models and integrate the knowledge into one model, respectively. The integrated model can be used directly for inference or for further fine-tuning. We conduct extensive experiments on various datasets for recommendation and language tasks, and the results show that Compatibility-aware Knowledge Integration can effectively optimize incompatible parameters under multiple tasks and settings to break through the training limit of the original model without increasing the inference cost.

==> tex/6limitation.tex <==
\section*{Limitation}

Dynamic role allocation mechanism proposed by our Bidirectional Enhanced Learning framework (\methodbrief{}) is effective, but costs more than only training the LLMs and SRMs. Although it is not so important in the most cases.

==> tex/999aaai_checklist.tex <==
\section*{Checklist}

\begin{enumerate}
\item This paper:
    \begin{enumerate}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced \answerYes{Yes}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results \answerYes{Yes}
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper \answerYes{Yes}
    \item Does this paper make theoretical contributions? \answerYes{Yes}
    \end{enumerate}

\item If yes, please complete the list below.
    \begin{enumerate}
    \item All assumptions and restrictions are stated clearly and formally. \answerYes{Yes}
    \item All novel claims are stated formally (e.g., in theorem statements). \answerYes{Yes}
    Proofs of all novel claims are included. \answerYes{Yes}
    \item Proof sketches or intuitions are given for complex and/or novel results. \answerYes{Yes}
    \item Appropriate citations to theoretical tools used are given. \answerYes{Yes}
    \item All theoretical claims are demonstrated empirically to hold. \answerYes{Yes}
    \item All experimental code used to eliminate or disprove claims is included. \answerYes{Yes}
    \item Does this paper rely on one or more datasets? \answerYes{Yes}
    \end{enumerate}

\item If yes, please complete the list below.
    \begin{enumerate}
    \item A motivation is given for why the experiments are conducted on the selected datasets \answerYes{Yes}
    \item All novel datasets introduced in this paper are included in a data appendix. \answerYes{Yes}
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \answerYes{Yes}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \answerYes{Yes}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \answerYes{Yes}
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \answerYes{Yes}
    \item Does this paper include computational experiments? \answerYes{Yes}
    \end{enumerate}

\item If yes, please complete the list below.
    \begin{enumerate}
    \item Any code required for pre-processing data is included in the appendix. \answerYes{Yes}.
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. \answerYes{Yes}
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \answerYes{Yes}
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from \answerYes{Yes}
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \answerYes{Yes}
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \answerYes{Yes}
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \answerYes{Yes}
    \item This paper states the number of algorithm runs used to compute each reported result. \answerYes{Yes}
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \answerYes{Yes}
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \answerYes{Yes}
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \answerYes{Yes}
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \answerYes{Yes}
    \end{enumerate}
\end{enumerate}
